Prescriptive Process Monitoring Under Resource Constraints: A Causal Inference Approach

Prescriptive process monitoring is a family of techniques to optimize the performance of a business process by triggering interventions at runtime. Existing prescriptive process monitoring techniques assume that the number of interventions that may be triggered is unbounded. In practice, though, specific interventions consume resources with finite capacity. For example, in a loan origination process, an intervention may consist of preparing an alternative loan offer to increase the applicant's chances of taking a loan. This intervention requires a certain amount of time from a credit officer, and thus, it is not possible to trigger this intervention in all cases. This paper proposes a prescriptive process monitoring technique that triggers interventions to optimize a cost function under fixed resource constraints. The proposed technique relies on predictive modeling to identify cases that are likely to lead to a negative outcome, in combination with causal inference to estimate the effect of an intervention on the outcome of the case. These outputs are then used to allocate resources to interventions to maximize a cost function. A preliminary empirical evaluation suggests that the proposed approach produces a higher net gain than a purely predictive (non-causal) baseline.

==> sections/RelatedWork.tex <==
\section{Related Work} \label{sec:relatedwork}
In this section, we discuss the essential preliminaries that we should know before introducing our approach. Additionally, we will show the related work to this paper. 


\todo[inline]{To be completed}

%\subsection{Preliminaries}
%The core of any outcome-oriented predictive or prescriptive process monitoring is the event log, representing the execution of any business process, e.g., \textit{loan application}. An event log is a set of complete traces where each one consists of a sequence of events. Each event belongs to the same business case and carries information at least about (i) activity: (describes what happened?), e.g., apply, complete an application, etc. (ii) timestamp: (indicates when an activity occurred?). (iii) resource: (who did the work?), e.g., user 1, user 2, etc. Furthermore, additional information related to case attributes, e.g., the client's age \cite{teinemaa2019outcome}. In the following, we define some terms that we will use to build our approach during this paper. \\


